Attacking Image Splicing Detection and Localization Algorithms Using Synthetic Traces

Recent advances in deep learning have enabled forensics researchers to develop a new class of image splicing detection and localization algorithms. These algorithms identify spliced content by detecting localized inconsistencies in forensic traces using Siamese neural networks, either explicitly during analysis or implicitly during training. At the same time, deep learning has enabled new forms of anti-forensic attacks, such as adversarial examples and generative adversarial network (GAN) based attacks. Thus far, however, no anti-forensic attack has been demonstrated against image splicing detection and localization algorithms. In this paper, we propose a new GAN-based anti-forensic attack that is able to fool state-of-the-art splicing detection and localization algorithms such as EXIF-Net, Noiseprint, and Forensic Similarity Graphs. This attack operates by adversarially training an anti-forensic generator against a set of Siamese neural networks so that it is able to create synthetic forensic traces. Under analysis, these synthetic traces appear authentic and are self-consistent throughout an image. Through a series of experiments, we demonstrate that our attack is capable of fooling forensic splicing detection and localization algorithms without introducing visually detectable artifacts into an attacked image. Additionally, we demonstrate that our attack outperforms existing alternative attack approaches. %

==> intro_v0.tex <==
Image splice detection and localization algorithms are becoming imperative to fight against the falsified images across the internet world, as the image editing and generating techniques become more and more popular and accessible to the public. Recently the multimedia researchers have developed multiple techniques to fight against the falsified images, among them the deep learning based architecture shows their advance in performance. 



One type of approach of the state-of-the-art algorithms are utilizing the siamese convolutional neural network(CNN) to extract and compare the forensic features of an image. These algorithms are designed to extract the forensic features left by the before and post processing operation of an image. With the assumption that different parts of a pristine image should undergo the same processing operation and shows the same forensic features, while spliced image should shows the difference over forensic features between pristine and splice regions with different processing operation. These siamese network based algorithms have gained much popularity since they don't require prior knowledge of a potential falsified image. Once get trained, these siamese network based algorithms can easily applied to the wild images.



However, recent researches have also shown the weakness of the neural networks and the corresponding algorithms by launching adversarial attacks. One of the most popular types of attack is the adversarial examples. Adversarial examples utilize the output of one or more layers of the target neural network to construct the loss functions, then back propagate the corresponding gradients into the input images. Researchers have utilize this technique to successfully attack many neural-network-based algorithms. The other type would be the GAN-based attack. For example, researchers have also shown that the attacker can use a generative neural network to attack against the image forensic networks.

Since the recent advanced algorithms also use siamese structure of neural network to perform splice detection and localization, it is also worthwhile to demonstrate the weakness of such algorithm by studying the corresponding adversarial attack. Some researchers have already developed the adversarial attack on these splice detection or localization algorithms using adversarial examples. However, adversarial examples against them could still shows shortage. First, some of the siamese-based neural network, on which the splice detection and localization algorithms are relying, only accept a specific input size, Therefore the adversarial examples cannot attack any image with a smaller size then the input of the siamese-based network. Second, these algorithms might also use image patch sampling method over the full-size image. Thus the performance of the adversarial examples on the these algorithms might fluctuate up and down, depending on different strategy of image patches sampling. Third, these attack cannot attack multiple algorithms simultaneously, and also shows weak transferability between different algorithms. In such case, investigator can defend the splice detection and localization algorithms by simply combine the results of different algorithms together.   

To solve the problem and establish an efficient and general adversarial attack on both the splice detection and localization algorithms, in this paper, We propose a new attack that can remove the difference of forensic features in the splice images. This attack consists of two training phase. In the phase 1 we pre-train the generator to learn to generate forensic features for an image. In the phase 2 we train the generator to fool the specific target siamese networks of the algorithms. At last we use the trained generator to attack the splice image in once, regardless of the strategy of splitting images as well as training specifically for each image. After the attack, the splice detection algorithms cannot discriminate between splice and pristine images, and the splice localization algorithms are not be able to localize the correct falsified region. Generally, the main contributions of this paper are:

\begin{itemize}
\item
We show that the current state-of-the-art forensic detection and localization algorithms are vulnerable to adversarial attack 
\item
We propose a new attack that can remove the difference of forensic features between the spliced and authentic regions of the images by synthesizing new forensic traces.
\item
The perturbation introduced by our proposed attack is invisible to the human eyes, therefore investigators are not able to discriminate the attack by their own judge.
\item
Our proposed attack can generate spatially even and content-related noise patterns, therefore it is insensitive to different sampling method of the splice detection and localization algorithms.  
\item 
Our proposed attack can attack several algorithms simultaneously.
\item
Our proposed attack shows a good transferability in attacking the unseen algorithms.
\item 
Our proposed attack is generative, which means the attacker doesn't need to retrain for every image. Also, it can be adapted to any images with sizes larger than $11\times11$.
\end{itemize}

By multiple experiments and comparisons, we demonstrate that our proposed attack can fool the splice detection and localization algorithms, with only introducing invisible pixel perturbations and remains high image quality.



==> results_v1.tex <==
After the training process, we get the final $G$ as our generator. This Generator is capable to attack both the Forensic Similarity Matrices and the EXIF-SC in both forgery detection and localization tasks. It can also transfer to the Noiseprint, with no prior knowledge. To demonstrate that, in the following subsections, we first show the results of patch-wise successful attack rate (SAR) of each similarity network. Second, we evaluate how well our attack performs on forgery detection. Third, we show the performance of our attack by comparing the localization scores between non-attacked and attacked images. At last we also show the ability of our attack on the Noiseprint that is "unseen" to the generator. We use the Camera Model dataset for the evaluation on patch-wise attack performance, and the Columbia Database~\cite{}, the Carvalho DSO-1 Database~\cite{} and the Korus Real Time Database~\cite{} for splice detection and localization evaluations.

\subsection{Evaluation Matrices}
To evaluate our proposed method, We utilize several matrices, to quantitatively measure the performance of our proposed method. 

\subsubsection{Image Quality}
We use two index to measure the output images quality: the PSNR~\cite{} and the SSIM~\cite{}, by comparing the attacked images with the original images. We note that the overall goal of the attack is to synthesize the forensic trace, which is invisible to human eyes, to fool the target algorithms. But not to get a very high PSNR and SSIM score. Thus the image quality is a rough measurement to help us evaluate about how visible the synthesized trace is. Therefore, a good attack only need to achieve an acceptable image quality.

\subsubsection{Patch-wise attack Performance}
For directly evaluating performance of the patch-wise attack on siamese networks, we compare between the original mis-classification rate(OMR) as the baseline performance, with the successful attack rate(SAR). Both the OMR and the SAR can be defined as 

\begin{equation}
\label{SAR}
OMR / SAR = \frac{N^{+}}{N}
\end{equation}

Where the nominator $N^{+}$ represents the number of pair of evaluated patches from different sources to be classified as "similar" by the siamese network, and the denominator $N$ is the total number of pairs of evaluated patches from different sources. The only difference is that the OMR is computed using the original image patches while the SAR is computed using the attacked image patches. By comparing the OMR and the SAR, we can quantitatively measure the $G$'s ability of synthesizing forensic traces to fool the siamese networks.

\subsubsection{Splice Detection}
Next, For evaluating the performance of the attack on splice detection, We use the mAP(mean average precision, which is equivalent to the AUC of the ROC curve) to evaluate the performance of the proposed attack. We note that for the splice detection task, the mAP have three important milestones. First, when the mAP equals to 1, it means that the detector can always successfully detect the splice image. Second, when the mAP equals to 0.5, it means that the detector can not discriminate between the spliced and the authentic images, and can only make random guess. Last, then the mAP equals to 0, it means the current detector can only able to predict all images, including both the spliced and the authentic images, to be authentic. 

\subsubsection{Splice Localization}
At last, For measure the performance of the attack on splice localization, we use the F-1 and the Matthews correlation coefficient (MCC) scores for the pixel-level evaluation. They are defined as: 

{\footnotesize
\begin{align}
&F_{1} = \frac{2 \times Precision \times Recall}{Precision + Recall}\\
&MCC = \frac{TP \times TN - FP \times FN}{\sqrt{(TP + FP)(TP+FN)(TN+FP)(TN+FN)}}
\end{align} 
}%

Besides, for the threshold method that the localization method to achieve the prediction mask, we adapt the per-image thresholding method. This is the ideally perfect scenario for the investigator. In such case the investigator will analysis the prediction map by selecting multiple level of threshold, then choose the most probable result by personal judgment. Therefore it would be the best possible localization performance made by the investigator.

\subsection{Performance of Attack on Image Patches}

\begin{table*}
\caption{Image Patch level performance of the proposed attack}
\label{table: PatchPerformance}
\small
\centering
\setlength{\tabcolsep}{1.5 mm}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
 \multirow{2}{*}{Training $S_{n}$} & \multirow{2}{*}{Siamese Network} & \multicolumn{4}{c|}{Seen Models} & \multicolumn{4}{c|}{Unseen Models}\\
 \cline{3-10}
 & & m-OMR & m-SAR & m-PSNR & m-SSIM & m-OMR & m-SAR & m-PSNR & m-SSIM\\
 \hline
 FSM & \multirow{4}{*}{FSM} & 6.9\% & 99.9\% & 45.2 & 0.991 & 7.2\% & 99.9\% & 45.2 & 0.991 \\
 \cline{1-1}\cline{3-10}
 EXIF-SC & & 6.9\% & 34.9\% & 42.5 & 0.981 & 7.2\% & 35.8\% & 42.5 & 0.981 \\
 \cline{1-1}\cline{3-10}
 Both, No Init & & 6.9\% & 99.9\% & 40.9 & 0.975 & 7.2\% & 99.9\% & 40.9 & 0.975 \\
 \cline{1-1}\cline{3-10}
 Both & & 6.9\% & \bf{99.9\%} & 41.3 & 0.976 & 7.2\% & \bf{99.9\%} & 41.4 & 0.976\\
 \hline 
 FSM & \multirow{4}{*}{EXIF-SC} & 13.6\% & 15.6\% & 45.2 & 0.991 & 14.3\% & 16.4\% & 45.2 & 0.991 \\ 
 \cline{1-1}\cline{3-10}
 EXIF-SC & & 13.6\% & 96.3\% & 42.5 & 0.981 & 14.3\% & 96.2\% & 42.5 & 0.981 \\
 \cline{1-1}\cline{3-10}
 Both, No Init & & 13.6\% & 97.0\% & 40.9 & 0.975 & 14.3\% & 97.1\% & 40.9 & 0.975 \\
 \cline{1-1}\cline{3-10}
 Both & & 13.6\% & \bf{97.4\%} & 41.3 & 0.976 & 14.3\% & \bf{97.5\%} & 41.4 & 0.976\\
 \hline
\end{tabular}
\end{table*}

We first evaluate the ability of our attack directly to the $S_{n}$s. Based on our database, we use the test set of both Group A (Seen models) \& B (Unseen models) to evaluate the successful attack rate(SAR) in patch level. In total, for the test set we have 14,4000 128$\times$128$\times$3 image patches from group A and 40,000 image patches from group B. To generate pairs of patches that from different sources, we first shuffle the test set of each camera model, than pairing the image patches and randomly selected 8,000 pairs for every combination of two camera models. This results in 1,224,000 pairs from the group A and 80,000 pairs from the group B. 

The detail results of four training strategies of our attack is shown in Table~\ref{table: PatchPerformance}. The best SAR scores of each evaluated siamese network are marked in bold face. The result shows that first, the proposed attack can fool the Forensic similarity matrices (mark as FSM), the EXIF-SC and even both of them simultaneously. Second, the attack on the FSM slightly transfer to the attack on the EXIF-SC, but the attack on the EXIF-SC transfer more strongly to the FSM. Third, when we attack two siamese networks together, we can achieve a higher or equal SAR than to attack only on one of them. At last, we can also see that training against both siamese network with phase I initialization increases the patch level SAR for attacking both $S_n$s.

\subsection{Image Quality over Three Evaluation Database}
\begin{table}
\caption{Image quality, with different training $S_n$}
\label{table: quality}
\small
\centering
\setlength{\tabcolsep}{1.0 mm}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 \multirow{2}{*}{Training $S_{n}$} & \multicolumn{2}{c|}{Columbia} & \multicolumn{2}{c|}{DSO-1} & \multicolumn{2}{c|}{Korus RT}\\
 \cline{2-7} &PSNR&SSIM&PSNR&SSIM&PSNR&SSIM\\
 \hline
 FSM & 44.75 & 0.987 & 43.74 & 0.984 & 43.98 & 0.985 \\
 \hline
 EXIF-SC & 42.84 & 0.981 & 41.79 & 0.976 & 41.61 & 0.980 \\
 \hline
 Both, No Init & 41.63 & 0.975 & 40.86 & 0.967 & 40.97 & 0.973 \\
 \hline
 Both & 42.08 & 0.976 & 40.98 & 0.968 & 40.84 & 0.973 \\
 \hline
\end{tabular}
\end{table}

Next, we show the attacked image quality of Columbia, Carvalho DSO-1 and Korus RT databases in the Table.~\ref{table: quality}. The image quality is measured by mean PSNR and SSIM over the whole database. The attacked image from all three database have the mean-PSNRs higher than 40, and the mean-SSIMs higher than 0.96. Through this table, we show that our proposed attack can only introduce very small perturbation, which is invisible to human eyes. Therefore, the investigator cannot tell by eyes that if an image have been attacked.

\subsection{Performance of Attack on Splice Detection}
\begin{table}
\caption{Splice detection performance, measured by mAP}
\label{table: detection}
\small
\centering
\setlength{\tabcolsep}{1.5 mm}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|}
\hline
 \multirow{2}{*}{Training $S_{n}$} & \multirow{2}{*}{\shortstack{Detection\\Method}} & Columbia & DSO-1 & Korus RT\\
 \cline{3-5}
  & & \multicolumn{3}{c|}{m-AP}\\
 \hline
 Baseline & \multirow{5}{*}{FSM} & 0.94 & 0.93 & 0.67 \\
 \cline{1-1}\cline{3-5} 
 FSM & & 0.46 & 0.14 & 0.10 \\
 \cline{1-1}\cline{3-5} 
 EXIF-SC & & 0.89 & 0.89 & 0.65 \\
 \cline{1-1}\cline{3-5} 
 Both, No Init & & 0.47 & \bf{0.05} & \bf{0.06} \\
 \cline{1-1}\cline{3-5} 
 Both & & \bf{0.46} & 0.08 & 0.15 \\
 \hline
 Baseline & \multirow{5}{*}{EXIF-SC} & 0.98 & 0.76 & 0.54 \\
 \cline{1-1}\cline{3-5} 
 FSM & & 0.97 & 0.85 & 0.51 \\
 \cline{1-1}\cline{3-5} 
 EXIF-SC & & 0.57 & 0.07 & 0.11\\
 \cline{1-1}\cline{3-5} 
 Both, No Init & & \bf{0.32} & \bf{0.13} & 0.09 \\
 \cline{1-1}\cline{3-5} 
 Both & & 0.38 & 0.08 & \bf{0.09} \\
 \hline
\end{tabular}
\end{table}

The performances of the attack on splice detection, via four different training strategies, are listed in the Table.~\ref{table: detection}. Again, the lowest scores of each detection algorithms (with best attack performance) are marked in bold face. Here we evaluate two forgery detection algorithm based on different $S_{n}$s. The first is the Forensic similarity matrices (FSM) proposed by Mayer and Stamm~\cite{}, accompany with spectral clustering algorithm on the similarity scores over the analysis block grids. The second is the EXIF-SC proposed by Efros and Huh~\cite{}, which detects the splice content by measure the mean value of the mean-shift clustering results on analysis block grids.

This result proves that, first, our attack can successfully fool the state-of-the-art image splice detector. Second, the attack on the EXIF-SC transfers better than the attack on the FSM, which is consistent with the fact that the EXIF-SC is designed to learn not only the camera model features, but also other EXIF information. Third, Attack on both of them can achieve a higher performance. At last, though the both attack without the phase 1 pre-training has slightly advance than the one with phase 1 training, their performance are still in the similar level. We will also show the phase 1 training might have significant improvement in the localization and the transferability in the following sections.


\subsection{Performance of Attack on Splice Localization}

\begin{figure*}[!h]
\centering
\setlength{\fboxsep}{0pt}
\begin{minipage}[t]{1\textwidth}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/org_canong3_nikond70_sub_04.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/ground_true_canong3_nikond70_sub_04.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_org_misl_canong3_nikond70_sub_04.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_org_exif_canong3_nikond70_sub_04.jpg}}} 
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_org_np_canong3_nikond70_sub_04.jpg}}}
    \centerline{(a) Left to right: pristine image, ground truth mask, heat map of the FSM, EXIF-SC and Noiseprint}
    \smallskip
\end{minipage}
\begin{minipage}[t]{1\textwidth}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/atk_canong3_nikond70_sub_04.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/atk_distort_canong3_nikond70_sub_04.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_atk_misl_canong3_nikond70_sub_04.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_atk_exif_canong3_nikond70_sub_04.jpg}}} 
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_atk_np_canong3_nikond70_sub_04.jpg}}}
    \centerline{(b) Left to right: attacked image, perturbation, heat map of the FSM, EXIF-SC and Noiseprint}
    \smallskip
\end{minipage}
\begin{minipage}[t]{1\textwidth}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/org_nikond70_kodakdcs330_sub_21.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/ground_true_nikond70_kodakdcs330_sub_21.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_org_misl_nikond70_kodakdcs330_sub_21.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_org_exif_nikond70_kodakdcs330_sub_21.jpg}}} 
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_org_np_nikond70_kodakdcs330_sub_21.jpg}}}
    \centerline{(c) Left to right: pristine image, ground truth mask, heat map of the FSM, EXIF-SC and Noiseprint}
    \smallskip
\end{minipage}
\begin{minipage}[t]{1\textwidth}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/atk_nikond70_kodakdcs330_sub_21.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/atk_distort_nikond70_kodakdcs330_sub_21.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_atk_misl_nikond70_kodakdcs330_sub_21.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_atk_exif_nikond70_kodakdcs330_sub_21.jpg}}} 
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Columbia/heat_atk_np_nikond70_kodakdcs330_sub_21.jpg}}}
    \centerline{(d) Left to right: attacked image, perturbation, heat map of the FSM, EXIF-SC and Noiseprint}
    \smallskip
\end{minipage}
\caption{Attack examples on the Columbia Database. Here we display 2 attacked examples, each one occupy two rows of pictures. The row (a) and (c) contain the original spliced images, their corresponding ground truth masks and the splice localization heat maps predicted by all three algorithms. The row (b) and (d) contain the attacked images, the perturbation introduced by our attack and the predicted heat maps. Note that the perturbation on the images are scaled up for 10 times for better visualization.}
\hfill
\label{fig: ColumbiaExamples}
\end{figure*}

\begin{figure*}[!h]
\centering
\setlength{\fboxsep}{0pt}
\begin{minipage}[t]{1\textwidth}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/org_splicing-34.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/ground_true_splicing-34.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_org_misl_splicing-34.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_org_exif_splicing-34.jpg}}} 
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_org_np_splicing-34.jpg}}}
    \centerline{(a) Left to right: pristine image, ground truth mask, heat map of the FSM, EXIF-SC and Noiseprint}
    \smallskip
\end{minipage}
\begin{minipage}[t]{1\textwidth}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/atk_splicing-34.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/atk_distort_splicing-34.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_atk_misl_splicing-34.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_atk_exif_splicing-34.jpg}}} 
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_atk_np_splicing-34.jpg}}}
    \centerline{(b) Left to right: attacked image, perturbation, heat map of the FSM, EXIF-SC and Noiseprint}
    \smallskip
\end{minipage}
\begin{minipage}[t]{1\textwidth}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/org_splicing-89.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/ground_true_splicing-89.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_org_misl_splicing-89.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_org_exif_splicing-89.jpg}}} 
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_org_np_splicing-89.jpg}}}
    \centerline{(c) Left to right: pristine image, ground truth mask, heat map of the FSM, EXIF-SC and Noiseprint}
    \smallskip
\end{minipage}
\begin{minipage}[t]{1\textwidth}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/atk_splicing-89.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/atk_distort_splicing-89.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_atk_misl_splicing-89.jpg}}}
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_atk_exif_splicing-89.jpg}}} 
    \fbox{\includegraphics[width=0.19\textwidth]{{fig/L2/Carvalho/heat_atk_np_splicing-89.jpg}}}
    \centerline{(d) Left to right: attacked image, perturbation, heat map of the FSM, EXIF-SC and Noiseprint}
    \smallskip
\end{minipage}
\caption{Attack examples on the Carvalho DSO-1 Database. Again, we display 2 attacked examples, each one occupy two rows of pictures. The row (a) and (c) contain the original spliced images, their corresponding ground truth masks and the splice localization heat maps predicted by all three algorithms. The row (b) and (d) contain the attacked images, the perturbation introduced by our attack and the predicted heat maps. Note that the perturbation on the images are scaled up for 10 times for better visualization.}
\hfill
\label{fig: CarvalhoExamples}
\end{figure*}

\begin{table}
\caption{Splice localization performance, per image thresholds}
\label{table: LocalizationPerImg}
\small
\centering
\setlength{\tabcolsep}{1 mm}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
 \multirow{2}{*}{Training $S_{n}$} &\multirow{2}{*}{\shortstack{Localization\\Method}} & \multicolumn{2}{c|}{Columbia} & \multicolumn{2}{c|}{DSO-1} & \multicolumn{2}{c|}{Korus RT}\\
 \cline{3-8}
 & & F1 & MCC & F1 & MCC & F1 & MCC\\
 \hline
 Baseline & \multirow{5}{*}{FSM} & 0.90 & 0.86 & 0.84 & 0.82 & 0.41 & 0.39 \\
 \cline{1-1}\cline{3-8} 
 FSM & & 0.66 & 0.55 & 0.49 & 0.40 & 0.26 & 0.24 \\
 \cline{1-1}\cline{3-8} 
 EXIF-SC & & 0.82 & 0.77 & 0.65 & 0.60 & 0.37 & 0.37 \\
 \cline{1-1}\cline{3-8} 
 Both, No Init & & 0.71 & 0.60 & 0.49 & 0.41 & 0.25 & 0.23 \\
 \cline{1-1}\cline{3-8} 
 Both & & \bf{0.58} & \bf{0.44} & \bf{0.40} & \bf{0.30} & \bf{0.23} & \bf{0.22} \\
 \hline
 Baseline & \multirow{5}{*}{EXIF-SC} & 0.91 & 0.88 & 0.57 & 0.51 & 0.28 & 0.26 \\
 \cline{1-1}\cline{3-8} 
 FSM & & 0.90 & 0.87 & 0.52 & 0.46 & 0.26 & 0.26 \\
 \cline{1-1}\cline{3-8} 
 EXIF-SC & & 0.73 & 0.65 & 0.38 & 0.26 & 0.23 & 0.21 \\
 \cline{1-1}\cline{3-8} 
 Both, No Init & & \bf{0.62} & \bf{0.51} & 0.38 & 0.28 & 0.23 & 0.21\\
 \cline{1-1}\cline{3-8} 
 Both & & 0.66 & 0.55 & \bf{0.36} & \bf{0.25} & \bf{0.22} & \bf{0.20} \\
 \cline{1-1}\hline
 Baseline & \multirow{5}{*}{Noiseprint} & 0.81 & 0.74 & 0.75 & 0.72 & 0.33 & 0.32 \\
 \cline{1-1}\cline{3-8} 
 FSM & & 0.75 & 0.67 & 0.59 & 0.53 & 0.28 & 0.27 \\
 \cline{1-1}\cline{3-8} 
 EXIF-SC & & 0.76 & 0.68 & 0.64 & 0.59 & 0.34 & 0.32 \\
 \cline{1-1}\cline{3-8} 
 Both, No Init & & 0.75 & 0.68 & 0.50 & 0.42 & 0.27 & 0.26 \\
 \cline{1-1}\cline{3-8} 
 Both & & \bf{0.69} & \bf{0.59} & \bf{0.47} & \bf{0.37} & \bf{0.24} & \bf{0.22} \\
 \hline
\end{tabular}
\end{table}



To quantitatively illustrate the ability of our attack to fool the splice localization, we compare the localization performance of the algorithms before and after our attack. The per image thresholding results are shown in the table.\ref{table: LocalizationPerImg}. Again, the lowest scores of each localization algorithms, which means the highest attack performance, are marked in bold face. 

Unlike the detection tasks, which only predict if there exists an splice in the image, the splice localization algorithms will predict a potential splice region. In fact the splice localization methods always provide a visual illustration of the spacial distribution of the forensic traces over the full-size image for the investigator. The investigator can rely on the predict mask of the potential splice region, then compare between the mask with the image content, to determine if an image has been spliced. Because the clustering algorithms the localization algorithms uses might always clusters the image into two regions, even for the authentic image, it is nearly impossible, nor incorrect, to make the localization algorithms predict no splice region. Instead, a successful attack should make the predicted region has low correlation with the ground truth mask. Thus the investigator cannot tell the splice region by personal judgment.

For the results, both table shows that after our attack, the performance of all the three localization algorithms drop significantly. For a better visualization of our attack, we display two examples for each database to show the influence of our attack on the forensic traces distribution and the localization results in Fig~\ref{fig: ColumbiaExamples} and \ref{fig: CarvalhoExamples}. These quantitative statistic and visualization of our attack performance demonstrate the ability of our attack to fool the state-of-the-art splice localization algorithms. Similar to the result of splice detection, the attack on EXIF-SC transfer better than the attack on forensic similarity network. Attack both siamese networks can also improve the attack performance, as well as improving the ability of black box attack on Noiseprint. This might be because that the two siamese network provide different feature domain information to the generator. Attacking both of them can force the generator to learn a wider feature space. Therefore it transfer better to Noiseprint. Besides, the results shows the phase 1 pre-training not only improve the attack on localization, but also significantly improves the attack performance on zero-knowledge attack on Noiseprint.


